Leveraging Synthetic Data to Learn Video Stabilization Under Adverse Conditions

Video stabilization plays a central role to improve videos quality. However, despite the substantial progress made by these methods, they were, mainly, tested under standard weather and lighting conditions, and may perform poorly under adverse conditions. In this paper, we propose a synthetic-aware adverse weather robust algorithm for video stabilization that does not require real data and can be trained only on synthetic data. We also present Silver, a novel rendering engine to generate the required training data with an automatic ground-truth extraction procedure. Our approach uses our specially generated synthetic data for training an affine transformation matrix estimator avoiding the feature extraction issues faced by current methods. Additionally, since no video stabilization datasets under adverse conditions are available, we propose the novel VSAC105Real dataset for evaluation. We compare our method to five state-of-the-art video stabilization algorithms using two benchmarks. Our results show that current approaches perform poorly in at least one weather condition, and that, even training in a small dataset with synthetic data only, we achieve the best performance in terms of stability average score, distortion score, success rate, and average cropping ratio when considering all weather conditions. Hence, our video stabilization model generalizes well on real-world videos and does not require large-scale synthetic training data to converge.

==> sections/deleteme.tex <==
Video stabilization plays a central role to improve videos quality. Despite the substantial progress made by these methods, they were, mainly, tested under standard weather and lighting conditions, and may perform poorly under adverse conditions.
In this paper, we propose to use synthetic data to provide robustness across different weather conditions when training a synthetic-aware algorithm for video stabilization. We also present a novel rendering engine to generate the required training data with an automatic ground-truth extraction procedure and an approach that uses synthetic data for training an affine transformation matrix estimator and avoids the feature extraction issues faced by current methods.
Our video stabilization model generalizes well on real-world videos and does not require large-scale synthetic training data to converge. Additionally, since no video stabilization datasets under adverse conditions are available, we propose the novel VSAC105Real dataset for evaluation. We compare our method to five state-of-the-art video stabilization algorithms using two benchmarks.
Our results show that current approaches perform poorly in at least one weather condition, and, even training in synthetic data only, we achieve the best performance in terms of stability average score, distortion score, success rate, and average cropping ratio when considering all weather conditions.


==> sections/limitations.tex <==
\section{Limitations}
Although our approach achieved state-of-the-art results, it has a few limitations addressed in this section.

Our approach can be trained only on synthetic data and does not require real-world videos. While this is an advantage, our algorithm, however, cannot leverage real data. In future work, we are planning to generalize our method to real data, too.

Our method achieves interesting results under foggy weather conditions. However, it only attains adequate performance in other classes. Increasing the number of synthetic training samples did not boost the performance of our video stabilization method. The reason could be that our model has already learned how to estimate the affine transformation matrix, and any further training videos were not advantageous. 


==> sections/releated_work_long_version.tex <==
\section{Related Work}
%Our work utilizes synthetic data for the task of video stabilization. Thus, video stabilization and synthetic data generation literature is briefly reviewed in this section. 
\paragraph*{Video Stabilization.}
% Feature extractors \cite{lowe2004distinctive,bay2006surf} usually include three steps: feature detection, description and matching.  Fortunately, there are methods that can do video stabilization while reserving all the content of the frame called full-frame video stabilization methods~\cite{choi2020deep,liu2021hybrid}. However, the main drawback is giving slightly less stable results and requiring more computation time. 



%using optical flow for video stabilization
%check

% \EN{Remove this paragraph? --- In general, video stabilization approaches comprise three main stages: camera motion estimation, motion smoothing, and warping. Techniques using block-matching-based~\cite{morimoto1996fast}, pixel-based~\cite{grundmann2011auto,choi2020deep}, and feature-based~\cite{gleicher2007re,lee2009video,liu2011subspace} have been proposed to estimate the camera motion. For smoothing the camera motion, works have applied Gaussian low-pass filter~\cite{liu2011subspace}, and L1-norm optimization~\cite{grundmann2011auto} to improve the frame transition. At last, per-pixel warp fields~\cite{yu2020learning,yu2019robust} and per-frame warp fields~\cite{liu2021hybrid} are recent approaches to create the warping functions.}
%The camera motion estimations. Some of them are block-matching-based~\cite{morimoto1996fast}, pixel-based~\cite{grundmann2011auto,choi2020deep}, and feature-based~\cite{gleicher2007re,lee2009video,liu2011subspace}. At the same time, for camera motion smoothing there some works that used Gaussian low-pass filter~\cite{liu2011subspace}, and L1-norm optimization~\cite{grundmann2011auto}. On the other hand, some works utilize per-pixel warp fields~\cite{yu2020learning,yu2019robust} or per-frame warp fields~\cite{liu2021hybrid}. These methods can be categorized broadly into learning-based and non-learning based approaches. 

Video stabilization methods can be categorized broadly into learning-based and non-learning-based approaches. 
%
Non-learning-based video stabilization methods do not perform training. For instance, Grundmann~\etal~\cite{grundmann2011auto} stabilize the shaky camera trajectory using L1-norm optimization under constraints.
% The work of Grundmann et al. \cite{grundmann2011auto} is an example of non-learning based video stabilization. They stabilize the shaky camera trajectory using L1-norm optimization technique under certain constrains.
Their method minimizes the first, second, and third derivatives of the resulting camera path to compute a smooth camera trajectory composed of constant, linear, and parabolic segments. Similarly, 
% \EN{Drawbacks and benefits of using non-learning-base methods?} \EN{Only one reference in this category?}
% Thus, giving a more pleasant stabilized video.
Bradley~\etal~\cite{bradley2021cinematic} address the stabilization task as a constrained convex optimization problem. They solve the homography estimation by working in log-homography space, where they model it without loss of convexity. These non-learning-based methods stabilize videos without the need for training data to tune the model's parameters. However, they tend to give less pleasant results, can work only under predefined conditions, and the model's parameters must be tuned manually.

The learning-based approaches, for their turn, can be classified into unsupervised and supervised approaches.
Non-supervised video stabilization methods require training videos but no need for annotated pairs of shaky-stable videos. 
Deep Iterative FRame INTerpolation (DIFRINT)~\cite{choi2020deep} is an unsupervised learning-based approach that can be trained in an end-to-end manner. It can stabilize videos without cropping original frames. Essentially, this method utilizes the frame interpolation technique to synthesize middle frames for video stabilization.  
% choi2020deep,wang2018deep
Supervised learning approaches, on the other hand, require ground-truth data, which is the main limitation of applying them to video stabilization.
%is the problem of generating ground truth data. 
Some works approached this problem using a mechanical stabilizer to generate ground-truth stable videos with their shaky counterparts. As an example, StabNet~\cite{wang2018deep} followed this procedure, generating videos for training CNNs for video stabilization. The network learns a warping transformation of multi-grids given the shaky video frames and the previously stabilized ones. On the other hand, Liu~\etal~\cite{liu2021hybrid} apply a learning-based hybrid-space fusion to compensate for optical flow inaccuracy. They synthesize stabilized frames by fusing the warped content estimated from neighboring frames. They can stabilize frames without cropping them and with fewer visual artifacts. Yu~\etal~\cite{yu2020learning} learn to stabilize videos using optical flow. They compute the per-pixel warp field from the optical flow of the shaky video, allowing to better handle moving objects and occlusion.
% proposed using optical flow for video stabilization. They compute the per-pixel warp field from the optical flow of the shaky video. This method learns to stabilize videos using the optical flow allowing to better handle moving objects and occlusion. 
In contrast to the works of Yu~\etal~\cite{yu2020learning}, Ali~\etal~\cite{ali2020learning} proposed a full-frame supervised video stabilization method that does not require optical flow. Their novel pipeline for dataset generation uses a linearly moving window on high-resolution images.

Despite the substantial progress made by these methods, they present a partial solution to the video stabilization problem since it is assumed that they will work under normal weather conditions and sufficient illumination. Finding resilient features in adverse conditions is rather challenging. For example, rain particles, foggy weather conditions, and low illumination pose clear challenges to finding robust features. Thus, it leads to inaccurate motion estimation and low-quality video stabilization. At the same time, collecting diverse real-world videos for training video stabilization methods is cumbersome and time-consuming. Moreover, generating data with perfect ground truth is not feasible given the physical limitation of recording the same scene from the same perspective via steady and shaky cameras.  

Our video stabilization method belongs to the supervised learning-based category. However, unlike other methods, we use only synthetic data for training. To the best of our knowledge, this is the first work to utilize synthetic videos for video stabilization. No pre-training or fine-tuning on real data is required, and by using only a small-scale training dataset, our method is more robust than state-of-the-art methods. 
\paragraph*{Affine and Homography Transformation.}
Estimating the affine or homography transformation between two images are two common approaches to align one image to another. For that aim, there are three different ways to find these matrices. First, to apply a feature extractor (e.g., SIFT, ORB, SURF, and OAN) to find resilient matching points between the two images. Then, to use outlier rejection algorithm (e.g., RANSAC and MAGSAC) to refine the selected pairs and to estimate the required transformation. Second, there are unsupervised methods to estimate the homography matrix~\cite{zhang2020content}. Third, there supervised methods~\cite{detone2016deep} that can be used to estimate the homography matrix, too.  

Although the traditional approach i.e. feature extraction one does well at standard conditions, it perform poorly under challenging conditions such as adverse weather conditions and low illumination. At the same time, supervised approaches cannot reflect scene parallax~\cite{ye2021motion} and generating a suitable training data is rather hard. On the other hand, unsupervised approaches elevated these problems but still it fails under large baseline alignment which makes it unpractical for applications such as image stitching and video stabilization. 

Unlike the previous methods, we learn the affine transformation in a supervised manner using specially generated synthetic training data for this task. Our method does not rely on real data. Additionally, it can be trained on unlimited number of training samples covering wide set of challenging scenarios such as heavy snow, dense foggy, and low illumination.
Estimating the affine transformation is of a special importance in video stabilization because it allows us to recover the camera translation, rotation and scale. Then, to apply other algorithms to smooth the camera transitions over the frames. While, it is possible to decompose the homograph matrix to extract these information, it is not accurate. At the same time, training a model to estimate the affine transformation is much more easier compared to estimating the the homography transformation.  
\paragraph*{Synthetic Data Generation.}
%synthetic data
Although the exponential increase in the amount of digital data today makes data collection easier than before, manual labelling of large volumes of examples with high quality and accurate labels still requires too much effort and comes with a high cost. The use of synthetic data in the computer vision community has shown to be a promising solution to overcome the lack of suitable data for training supervised learning models. Its increase in popularity started to attract many researchers to propose novel algorithms to generate such datasets with their corresponding ground truths. %Although special care needs to be taken to weigh each method’s advantages and disadvantages, they seem a promising solution to overcome the lack of suitable data for training supervised learning models.

Adapting a specific video game to generate synthetic data with its corresponding ground-truth for the task of semantic segmentation was presented by Richter~\etal~\cite{richter2016playing}, who modified the game Grand Theft Auto V for that purpose. They have shown that integrating synthetic and organic datasets in the training process for semantic segmentation improves the overall performance considerably. 
At the same time, another work by Shafaei~\etal~\cite{shafaei2016play} investigated the use of photo-realistic video games to generate synthetic data and their corresponding ground truths for image segmentation and depth estimation.
% Conducting many experiments, they proved that training a Convolutional Neural Network (CNN) using only synthetic data achieves a similar performance as with training on real data. 
Using open-source animation movies was another approach discussed by Butler~\etal~\cite{butler2012naturalistic}, who showed how to obtain an optical flow large-scale dataset, MPI-Sintel, following a systematic and easy process. Dosovitskiy~\etal~\cite{dosovitskiy2017carla} presented CARLA, a popular open-source simulator widely used for autonomous driving research. CARLA is built as an additional layer on Unreal Engine \cite{UnrealGameEngine}. It supports different weather types and two illumination conditions. The CARLA simulator can also provide ground-truth data for semantic segmentation and depth estimation tasks.
Recently, the UrbanScene3D simulator was proposed by Liu~\etal~\cite{liu2021urbanscene3d} and developed for computer vision and robotics research. The system supports autonomous driving and flying research in different environments. It is built on the Unreal Engine \cite{UnrealGameEngine} and AirSim \cite{shah2018airsim}. GANcraft is another work by Hao~\etal~\cite{hao2021gancraft} for generating photorealistic images. GANcraft can produce consistent images from different viewpoints without the need for paired ground-truth real images. GANcraft also allows controlling certain features of the generated images by leveraging style-conditioning images.

%Unfortunately, 
% Despite the great advancements of the previous simulators, they present a partial solution for the data generation issue because of the lack of control on the environmental elements. In addition, integrating new elements or behaviours to the scene, like new 3D model, material, or texture, is hard or unattainable. Moreover, these systems are limited to specific computer vision tasks. Although these approaches are based on high quality and rich 3D virtual worlds, the failure of such methods to randomize the scene elements will lead to some clear repetitions (to scene elements) when a large-scale dataset is required to be generated by these methods. Procedural synthetic data generation offers an alternative to the previous solution.
% In our system, we utilize Procedural Content Generation (PCG) to generate 3D virtual worlds. Thus, it can generate a special training data for the task of video stabilization. 
In our experiments, we show that generating accurate, appropriate training data and creating a pipeline that utilizes synthetic data can achieve superior results. Our model can still generalize to real videos even though our engine does not generate state-of-the-art photo-realistic videos.
